From Cross-Modal to Mixed-Modal Visible-Infrared Re-Identification

Visible-infrared person re-identification (VI-ReID) aims to match individuals across different camera modalities, a critical task in modern surveillance systems. While current VI-ReID methods focus on cross-modality matching, real-world applications often involve mixed galleries containing both V and I images, where state-of-the-art methods show significant performance limitations due to large domain shifts and low discrimination across mixed modalities. This is because gallery images from the same modality may have lower domain gaps but correspond to different identities. This paper introduces a novel mixed-modal ReID setting, where galleries contain data from both modalities. To address the domain shift among inter-modal and low discrimination capacity in intra-modal matching, we propose the Mixed Modality-Erased and -Related (MixER) method. The MixER learning approach disentangles modality-specific and modality-shared identity information through orthogonal decomposition, modality-confusion, and ID-modality-related objectives. MixER enhances feature robustness across modalities, improving cross-modal and mixed-modal settings performance. Our extensive experiments on the SYSU-MM01, RegDB and LLMC datasets indicate that our approach can provide state-of-the-art results using a single backbone, and showcase the flexibility of our approach in mixed gallery applications.

==> cvpr24/preamble.tex <==
%
% --- inline annotations
%
\usepackage[dvipsnames]{xcolor}
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}



==> sec/1_intro-old.tex <==
\section{Introduction}
\label{sec:intro}


Visible-infrared (VI) person re-identification (ReID) is an essential component of surveillance systems, designed to match individuals across different camera views under varying lighting conditions. Traditional VI ReID methods typically focus on cross-modality matching, where infrared/visible images serve as the query and visible/infrared images constitute the gallery. These methods primarily compute cross-modality matching scores between day and night images or vice versa. However, real-world scenarios require a system that operates seamlessly across all times of the day, accommodating cross-modal (infrared-to-visible) matching at night and uni-modal (visible-to-visible or infrared-to-infrared) matching during the day.
== general challenges V-I ReID

Current cross-modal VI ReID techniques primarily extract global representations \cite{Wang_2019_ICCV_AlignGAN, kniaz2018thermalgan, all-survey, Bi-Di_Center-Constrained, hetero-center, park2021learning} or local part-based representations through techniques like horizontal striping\cite{DDAG,cmSSFT} or attention mechanisms \cite{part1,wu2021Nuances}. Although these representations can be discriminative, they do not adequately address modality-specific discrepancies, leading to less robust modality-free features. 
To address these issues, recent methods focus on extracting modality-invariant features by disentangling them from modality-specific information \cite{HI-CMD, paired-images2, cmSSFT, zhu2023information, zheng2019camera, lu2024disentangling, shape-Erase23}. Some generative techniques \cite{HI-CMD, paired-images2, cmSSFT} aim to separate content information from modality-related style attributes. However, generating synthetic images can result in the loss of identity-related information. Some approaches \cite{zhu2023information, zheng2019camera} reconstruct features while enforcing orthogonality between modality-specific and modality-invariant information, but challenges remain in ensuring erased features do not retain modality-specific elements.
Shape information is leveraged in \cite{lu2024disentangling,shape-Erase23} to disentangle body-shape information from modality-aware identity information to make the extracted feature not dependent on shape. Although this method improves the matching performance, it needs extra information that is not available for all existing data, and erasing shape information from final features does not guarantee the absence of modality-specific information.

%== transition for mixed-modality

= Challenge: 

- With cross-modal I-V ReID,  we need 2 backbones, one for each cross-modal direction. This is too expensive  

- when we train one backbone with SOA methods, they do not perform as well in more realistic, etc...

== In this paper we focus on mixed-modality scenarios.

This paper addresses the above limitations in mixed-modal scenarios by proposing a \textbf{M}odality-\textbf{E}rased and Modality-\textbf{R}elated \textbf{I}D-discriminative mi\textbf{X} learning framework that 
features and Mixing, enhancing. 
Our model aims to learn discriminative information by identifying modality-related information that discriminates the foreground and then erases them from modality-shared information to purify them from modality-related information. Modality-related information must represent input objects by using attributes that are accessible and unique only in the modality. For example, in the VI person ReID problem, as illustrated in Fig. \ref{fig1:venn},  the information discriminating the person (foreground) from the background and other persons can be viewed as two parts: modality-specific and modality-shared information. The model should extract them from modality-shared information to have a robust feature representation for matching against modality change. Furthermore, we propose enhancing current methods by extracting identity-aware information and disentangling it into modality-related and modality-erased features. Since modality-related information is often more discriminative and unique for each individual, our method leverages this for mixed-modal matching. This strategy benefits the model in two ways: 
\begin{enumerate}
    \item By computing similarity between instances of the same modality, and
    \item By enhancing cross-modal matching performance, modality-erased features are more robust. %against modality changes.
\end{enumerate}

% In our \NM method, we train two modality-specific branches to extract the Visible and Infrared ID-aware features and propose a way to erase them from the shared breach by reversal gradient layer for improving cross-modal matching. Also, this part is beneficial for improving the accuracy of intra-modal or a mixture of modalities matching scenarios. 

For evaluation of our method, we analyze the concept of a Mix-Modality gallery problem, where the ReID system must handle various scenarios based on the time of day and modality. The Mix V-I ReID task presents significant challenges, as it involves matching individuals based on cross-modal images with substantial appearance differences (e.g., infrared versus visible) while also accurately distinguishing between individuals with minimal appearance differences within the same modality. Therefore, the model must differentiate between individuals irrespective of the modality and extract modality-invariant features to ensure accurate and unbiased person identification.
Our evaluation system measures the robustness of learned features against changes in modality, camera, and identity for existing VI ReID methods.






% These settings are designed to test the system's ability to handle diverse real-world scenarios, ensuring a robust evaluation of the proposed ReID system.

%cross-modal methods and %%%Disentaglment


% While these methods make the extracted identity-discriminative features robust against other disentangled information, selecting the appropriate information to erase is crucial. For instance, erasing shape information from final features does not guarantee the absence of modality-specific information. 
% To address
% Moreover, modality-specific information can be divided into two parts: background information or identity-aware attributes unique to one modality. Thus, to address this issue, identity-aware features must be separated from modality-specific ones.

%Disentanglement of features typically is characterized by the suppression of redundant features and amplification of relevant features. This implies that the identification of features that require to be suppressed is critical. Modality information in features often gets inherently entangled, even after attempts to disentangle features (needs reference), and so far, no work proposes a method to selectively suppress modality-related information, from identity-related features.

%main idea
% Alongside the Mix-Modality gallery settings, we propose a method to address the cross-modal and mix-modal problem by erasing proper identity-related modality-specific information from identity-related modality-invariant information, making these features robust against modality. Our model aims to identify appropriate modality-related information that discriminates the foreground and then erases them from modality-shared information to purify them from any modality-related information. Modality-related information must represent input objects by using attributes that are accessible and unique only in the modality. For example, in VI person ReID problem, as illustrated in Fig. \ref{fig1:venn},  the information discriminating the person (foreground) from the background and other persons can be viewed as two parts: modality-specific and modality-shared information. To have a robust feature representation for matching against modality change, the model should extract them from modality-shared information. In our \NM method, we train two modality-specific branches to extract the Visible and Infrared ID-aware features and propose a way to erase them from the shared breach by reversal gradient layer for improving cross-modal matching. Also, this part is beneficial for improving the accuracy of intra-modal or a mixture of modalities matching scenarios. 

Our main contributions are summarized as follows. \\
%(1) Defining the mixed-matching setting that is found in real-world scenarios. 
\noindent \textbf{(1)} A modality-erased feature learning paradigm is introduced for V-I ReID that separates modality-erased features from modality-identity-related ones through orthogonal decomposition and reversal gradient layer. Modality-identity-related features are guided by identity attributes specific to one modality. In contrast, modality-erased features are constrained to discover additional modality-shared discriminative semantic concepts, thereby explicitly enhancing the learned representation's diversity.\\
\noindent \textbf{(2)} Our modality-specific feature learning not only enhances the cross-modal matching performance but also makes intra-modality matching more robust than letting our ReID system be used in practical mix scenarios. Also, our learning approach is model agnostic, and it can be integrated into other SOTA methods. \\
\noindent \textbf{(3)} Multiple mixed-matching settings are defined based on real-world scenarios, and benchmark evaluations are performed on existing VI person ReID methods.
% \noindent \textbf{(3)} Based on the proposed modality-erased feature learning paradigm, we design a Modality-ID-Guided Diverse Feature Learning framework that jointly optimizes modality-related and modality-erased objectives to learn a modality-shared and discriminative integrated representation. Modality-identity-related information not only reinforces modality-erased information but is also utilized for matching in mixed or unimodal scenarios.\\
\noindent \textbf{(4)} Extensive experiments on the challenging SYSU-MM01 \cite{SYSU} and RegDB \cite{regDB} datasets indicate that our proposed BMDG strategy can outperform state-of-the-art methods for V-I person ReID. Additionally, our framework can be integrated into any part-based V-I ReID method, improving its performance for cross-modal retrieval applications.


%%%%% Local part-based fig1.b

\begin{figure}[t]
\centering
\includegraphics[width=0.9\columnwidth]{imgs/venn.png} % Reduce the figure size so that it is slightly narrower than the column. Don't use precise values for figure width. This setup will avoid overfull boxes.
\caption{The distribution of information in visible and infrared systems. The goal of the model is to extract robust features that discriminate the foreground from the background. This information can be considered as modality-erased or modality-related information.     }
\label{fig1:venn}
\end{figure}

In a multi-modal problem, the distribution of information about the desired object is divided into two parts: (a) Modality-erased and (b) modality-related. Both of them must discriminate the foreground. In cross-modal matching, the model needs to find robust modality-erased features that are shared between modalities and do not vary with the type of source information. 





% \begin{figure*}[t]
% \centering
% \includegraphics[width=0.9\textwidth]{imgs/compare.png} % Reduce the figure size so that it is slightly narrower than the column. Don't use precise values for figure width. This setup will avoid overfull boxes.
% \caption{An illustration of our motivation on VI-ReID. (Left) other methods: the extracted id-related features contain some information that is dependent on the modality, which degrades the performance in cross-modal matching. (Right)
% To make extracted features not biased on modality-specific information, we propose a modality-erased feature learning paradigm that decomposes the representation into modality-related features and modality-erased ones.     }
% \label{fig:com}
% \end{figure*}



==> sec/temp.tex <==
\section{Rationale}
\label{sec:rationale}
% 
%Having the supplementary compiled together with the main paper means that:
% 
%\begin{itemize}
%\item The supplementary can back-reference sections of the main paper, for example, we can refer to \cref{sec:intro};
%\item The main paper can forward reference sub-sections within the supplementary explicitly (e.g. referring to a particular experiment); 
%\item When submitted to arXiv, the supplementary will already included at the end of the paper.
%\end{itemize}
% 
%To split the supplementary pages from the main paper, you can use \href{https://support.apple.com/en-ca/guide/preview/prvw11793/mac#:~:text=Delete%20a%20page%20from%20a,or%20choose%20Edit%20%3E%20Delete).}{Preview (on macOS)}, \href{https://www.adobe.com/acrobat/how-to/delete-pages-from-pdf.html#:~:text=Choose%20%E2%80%9CTools%E2%80%9D%20%3E%20%E2%80%9COrganize,or%20pages%20from%20the%20file.}{Adobe Acrobat} (on all OSs), as well as \href{https://superuser.com/questions/517986/is-it-possible-to-delete-some-pages-of-a-pdf-document}{command line tools}.
% \\\\
Here is an explanation of how these metrics are calculated and what insights they provide about the performance of a ReID framework : 
\begin{itemize}
    \item \textbf{Cumulative Match Characteristics (CMC)}: These metrics provide a binary evaluation indicating, for each query image, whether a correct matching is within the top-k first matches. And, when we consider all the query images, we can calculate the percentage of correct matches found within the top-k ranked positions in the list of the retrieved images. This metric is particularly useful for assessing the ranking quality of the ReID model and showing how well the model can prioritize correct matches.  
    \item \textbf{Average Precision (AP)}: This metric considers all the retrieved gallery images for a given query image and calculates the average precision values at the positions where correct matches are found. Hence, a higher AP indicated that correct matches are consistently ranked near the top of the retrieval list.  
    \item \textbf{Mean Average Precision (mAP)}: This metric shows the overall ability of the model to rank correct matches higher in the retrieval list by averaging the AP values across all queries. 
    \item \textbf{Inverse Precision (INP)}: This metric focuses on the precision at the last position where a correct match is found. It measures how well the model can identify the hardest and final correct match for the query image. Therefore, a higher INP reflects the robustness of the model in identifying all potential matches.
    \item \textbf{Mean Inverse Precision (mINP)}: This metric complements the CMC and mAP, which are widely regarded as key metrics in the ReID task. It provides a comprehensive evaluation by averaging the INP values across all queries, thus indicating how well the least confident correct matches are identified accurately. 
\end{itemize} 

Together, these metrics provide a comprehensive understanding of the ReID system's effectiveness, offering insights into its performance across various challenging scenarios.

 \begin{figure}[!t]
        \centering
        \includegraphics[width=0.99\columnwidth]{imgs/Metrics.pdf} % Reduce the figure size to slightly narrower than the column. Don't use precise values for figure width. This setup will avoid overfull boxes.
        \caption{In the rank lists for Query 1 and 2 shown here, red and green denote incorrect and correct matches, respectively. Assuming there are seven correct matches in the gallery, Query 1 performs lower AP and INP results than Query 2. This is because, for Query 1, the correct matches are primarily found towards the bottom of the top-k ranks, whereas for Query 2, they are mostly found within the top ranks.}

        \label{fig1:venn_supp}
    \end{figure}

Next, we explain the reasoning behind the various case scenarios we have specially created for the SYSU-MM01 dataset: 

\textbf{Cross-Modal Baseline}: This scenario establishes the initial cross-modal baseline where the queries consist of IR images, while the gallery contains RGB images. To increase the matching difficulty, gallery images captured by camera ID 2 are excluded whenever query images originate from camera ID 3. Since cameras 2 and 3 both capture images in the same indoor location but in different modalities, this adjustment removes potential ``easy'' matches.    

- \textbf{Uni-modal}: We tested the two typical uni-modal scenarios :
\begin{itemize}
    \item  IR to IR: Matching IR images against other IR images. 
    \item  RGB to RGB: Matching RGB images against other RGB images.
\end{itemize} 
    
- \textbf{Mixed-Modal}: We created the mixed-modal case where queries are IR images and the gallery includes both IR and RGB images. And within this specific case, we implemented several scenarios :
\begin{itemize}
    \item  Baseline scenario: As described above, removing gallery RGB images taken at the same location as IR camera 3.
    \item  Scenario (*): Removed IR images from the gallery that share the same camera ID as the query image. This modification aims to simulate a more realistic ReID task, given that in most open-source datasets, the images are often captured within short time intervals from surveillance cameras, resulting in tracklets.
    
    \item  Scenario (**): Removed all the IR images from the gallery that match the ID of the query images. This specific scenario introduces negatives examples, hence adding complexity by including incorrect IR images. This enables us to assess how the model handles such false matches.
    \item  Scenario (***):   In this final scenario, all the IR images are removed from the gallery, reverting then to a cross-modal case.
\end{itemize}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.9\columnwidth]{imgs/Cases_Scenario.pdf} % Reduce the figure size so that it is slightly narrower than the column. Don't use precise values for figure width. This setup will avoid overfull boxes.
    \caption{The 4 different scenarios are illustrated here. From left to right, we have the baseline scenario (removing RGB images from camera 2 when IR image are taken camera 3), the second (*) scenario (removing all the IR images with the same camera ID as the query), then the (**) scenario (removing the IR gallery images of the same person captured by camera 3 \& 6), Finally the (***) scenario (removing all the IR images from gallery).}
    \label{fig1:venn}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.9\columnwidth]{imgs/Mode.pdf} % Reduce the figure size so that it is slightly narrower than the column. Don't use precise values for figure width. This setup will avoid overfull boxes.
    \caption{We want our framework consistent for all those matching modes.}
    \label{fig1:venn}
\end{figure}



==> tables/sysu-uni.tex <==
\resizebox{\linewidth}{!}{
\begin{tblr}{
  colspec={|l|ll|ll|ll|},
  cell{1}{1} = {r=2}{m},
  cell{1}{2} = {c=2}{c},
  cell{1}{4} = {c=2}{c},
  cell{1}{6} = {c=2}{c},
  hline{2} = {2-9}{},
  stretch = 0,
  colsep = 3.5pt
}
\hline
\textbf{Method} & \textbf{SYSU}(I$\rightarrow$I) &  & \textbf{SYSU}(V$\rightarrow$V) &  & \textbf{Market1501} &  \\
 & \textbf{R1} & \textbf{mAP} & \textbf{R1} & \textbf{mAP} & \textbf{R1} & \textbf{mAP} \\ \hline
DDAG\cite{DDAG} & 80.15 & 86.80 & 97.89 & 91.90 & 82.39 & 55.57 \\
MPANet\cite{wu2021Nuances} & 88.53 & 92.85 & 98.31 & 94.08 & 78.97 & 51.61 \\
DEEN \cite{LLCM} & 86.14 & 90.98 & 96.83 & 89.93 & 66.50 & 33.81 \\
SGEIL \cite{shape-Erase23} & 86.52 & 91.36 & 97.29 & 90.24 & 79.18 & 48.72 \\
SAAI \cite{SAAI} & 89.29 & 93.06 & 98.24 & 93.46 & 84.32 & 57.62 \\
IDKL\cite{IDKL} & 89.55 & 93.18 & 98.55 & 95.13 & 76.66 & 49.59 \\ \hline
\NM(E) & 90.18 & 93.65 & 98.13 & 93.50 & 82.90 & 56.56 \\
\NM(R) & 90.02 & 93.93 & 98.33 & 94.07 & 83.46 & 56.85 \\
\NM & \textbf{93.06} & \textbf{95.85} & \textbf{99.14} & \textbf{95.30} & \textbf{87.93} & \textbf{62.41} \\\hline\hline
Upper-bound & 88.06 & 92.80 & 98.85 & 95.20 & 96.17 & 86.24    \\
\hline
\end{tblr}
}

% \vspace{-0.3cm}
% \caption{Performance of techniques of V-I ReID trained by SYSU-MM01 dataset in Uni-modal matching settings on SYSU-MM01 and Market1501 dataset. The upper-bound is our baseline trained on SYSU-MM01 (Only I or V) and Market1501. (Other datasets are in Suppl. material).}
